SCVRL: Shuffled Contrastive Video Representation Learning

We propose SCVRL, a novel contrastive-based framework for self-supervised learning for videos. Differently from previous contrast learning based methods that mostly focus on learning visual semantics (e.g., CVRL), SCVRL is capable of learning both semantic and motion patterns. For that, we reformulate the popular shuffling pretext task within a modern contrastive learning paradigm. We show that our transformer-based network has a natural capacity to learn motion in self-supervised settings and achieves strong performance, outperforming CVRL on four benchmarks.

==> fig/overview.tex <==
\begin{figure*}
\begin{center}
\includegraphics[width=.99\columnwidth]{example-image-golden}
\hfill
\includegraphics[width=.99\columnwidth]{example-image-golden}
\end{center}
\caption{
% 
\textbf{Outline -- }
A figure summarizing the entire algorithm
}
\label{fig:overview}
% \vspace{-0.6cm}
\end{figure*}

==> fig/teaser.tex <==
\begin{figure}[t]
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
\includegraphics[width=\linewidth]{example-image-golden}
\end{center}
\caption{
% 
\textbf{Teaser -- }
Some nice summarizing image.
}
\label{fig:teaser}
\end{figure}

==> workshop/sec/3_method_bkp.tex <==
%!TEX root = ../main.tex
\section{Method}
\label{sec:method}
%
The goal of our approach is to better capture the temporal information inherent in videos in a self-supervised fashion. In Sec.~\ref{sec:visual_contrastive} we will first introduce a visual contrastive framework that yields robust spatial semantic features which acts as a strong baseline. Yet, it does not capture the temporal structures in videos. That is why we introduce in Sec.~\ref{sec:temporal_contrastive} our temporal contrastive objective to mitigate that. Lastly, in Sec.~\ref{sec:arch} we discuss our architecture and design choice for our framework. 
%
\subsection{Preliminaries on Contrastive Video Representation Learning (CVRL)}
\label{sec:preliminary}
% Recent work in self-supervised learning for images achieved impressive performance using contrastive learning~\cite{chen-simclr2020,he-moco2020,grill-byol2020}. 
The core idea in contrastive learning is to learn a representation space where similar samples are mapped close to each other, while dissimilar ones are far away. 

This representation is learned by an encoder $f$ using an InfoNCE contrastive loss \cite{oord-arxiv2018,he-moco2020} that operates over three inputs, a positive pair $x^a$ (anchor) and $x^p$ (positive) and a negative sample $x^a$, as follows:
\begin{align}
\mathcal{L}_{\text{contrastive}}&(f; x^a, x^p, x^{n_i}) = \\
&-\log \frac{e^{f(x^a) {\cdot} f(x^p) / \tau)}}{e^{f(x^a){\cdot}f(x^p) / \tau} + \sum_{i}^{N}e^{f(x^a){\cdot}f(x^{n_i}) / \tau}}, 
\label{eq:lv}
\end{align}


In this formulation, the encoder $f:\mathbb{R}^n \mapsto \mathcal{S}^{D-1}$, which maps data to $\mathbb{L}_2$ normalized feature vectors of dimension $D$. 

trained using the InfoNCE objective \cite{oord-arxiv2018,he-moco2020} 

with $\tau > 0$ the temperature parameter and $N \in \mathbb{Z}_+$ the number of negatives. In this paper, a sample is always a video clip of dimension $x \in \mathbb{R}^{T\times W\times H\times C}$ with $T$ the number of time frames, $W$ and $H$ spatial dimensions and $C$ color channels. 
One of the keys to produce rich representations lies in how the positive and negative samples are selected;




Empirically, positive pairs $x^a$ (anchor) and $x^p$ (positive), called anchor and positive respectively, are obtained by taking two independently randomly augmented versions of the same sample~\cite{bachman-neurips-2019, wu-instdisc2018, he-moco2019, chen-simclr2020}. 
Negatives$x^a$ (anchor) and $x^p$ (positive) are normally not explicitly sampled and extracted from the remaining samples in the batch. 

 for example, when the negatives are too simple, the network learns a trivial solution that is often uninformative for downstream tasks. While this sampling problem has been successfully explored in the image domain\cite{}\dvd{need citations here}, it remains rather unexplored in the video domain, where the temporal dimension $T$ carries new challenges. Next, we present a recent   sections we present a idea for sampling in videos that takes advantage of $T$ and uses that as a mean to \dvd{something} the learning. 
% Recent work in self-supervised learning for images achieved impressive performance using contrastive learning~\cite{chen-simclr2020,he-moco2020,grill-byol2020} (CL). The core idea of CL is learning a representation space $Z$ where samples from the same class are closer in the euclidean sense respect to samples from other classes. In particular, give two samples from the same class $z^a, z^p \in Z$, called respective anchor and positive, and a set of "negative" samples $z^{n_i} \in Z$, with $i \in \{1,...,N_v\}$, from a different class, we enforce the above constraint using the InfoNCE objective \cite{oord-arxiv2018,he-moco2020} 
% \begin{align}
% \mathcal{L}(z^a, z^p, z^{n_i}) = -\log \frac{\exp(z^a {\cdot}z^p / \tau)}{\exp(z^a{\cdot}z^p / \tau) + \sum_{i}^{N}\exp(z^a{\cdot}z^{n_i}  / \tau)}, 
% \label{eq:lv}
% \end{align}
% where $\tau$ is a temperature parameter. The value of the loss $\mathcal{L}$ is high when the distance between anchor and positive $z^a \cdot z^p$ is higher than the distance between anchor and negative $z^a \cdot z^n$. \\
% The representation space $Z$ is produced using a function $z = f(x)$ implemented as a deep neural network, which receives a sample $x$ in input and outputs a representation $z$. In this paper, a sample is always a video clip of dimension $x \in \mathcal{R}^{T\times W\times H\times C}$ with $T$ the number of time frames, $W$ and $H$ spatial dimensions and $C$ color channels. \\
% Provided this powerful framework, the key to produce a powerful unsupervised representation is the way positives and negatives are produced which is the core difference between recent methods. In the following section we will focus on this aspect or CL.
%
\subsection{Visual Contrastive Learning}
\label{sec:visual_contrastive}
CVRL~\cite{qian-cvrl2020} was the first work that adapted self-supervised contrastive learning from the image to the video domain. In this work, the positive pairs $x_{\scaleto{V}{4pt}}^a$ and $x_{\scaleto{V}{4pt}}^p$ are extracted by two independent temporally consistent spatial augmentations from two randomly chosen time steps of the same video. The negatives clips $x_{\scaleto{V}{4pt}}^{n_i}$ are produced by sampling from other videos. Given a network $f_{\scaleto{V}{4pt}}$ the visual contrastive objective can be written as
\begin{align}
\mathcal{L}_{\scaleto{V}{4pt}} = \mathcal{L}_{\text{contrastive}}(f_{\scaleto{V}{4pt}}; x_{\scaleto{V}{4pt}}^a, x_{\scaleto{V}{4pt}}^p, x_{\scaleto{V}{4pt}}^{n_i}).
\label{eq:lv}
\end{align}
This objective pulls together representations from the same video, while pushing away those from other videos. That ultimately leads to strong visual features, similar to the original contrastive objective in the image domain. However, it also naturally leads to temporal invariance since clips extracted from different time steps of a video are forced to be similar. This is sub-optimal for learning strong video representations especially when aiming at capturing temporal dynamics. For example, imagine videos in which a person is performing similar actions such as pulling and pushing. The only way to recognize the different actions is by paying attention to the order in which the frames are arranged. This would be impossible with a representation space learned with the above objective. To circumvent that, we propose a shuffled contrastive learning loss in the next section. 
% \dvd{I would extend here with an actual example. For example, in a video with action XYZ, understanding the dynamics (NJD and FDS) helps... XXX. It's going to be a rather trivial example, but it will immediately make the reader understand the problem. We need to emphasise this more!}
% 
% This framework can be adapted for videos, as suggested in~\cite{qian-cvrl2020}, by adding temporal jitterring to the augmentations for the positive pairs , as visualized in Fig.~\ref{fig:method}.
%
% A recent work that was instrumental to introduce CL for self-supervision in video representation is CVRL~\cite{qian-cvrl2020}. In this work, the positive clip $x^p$ is extracted from the same video of the anchor clip $x^a$ but at a different time point. On the other hand, the negatives clips $x^{n_i}$ are extracted from random videos. Given a network $f_v(\bullet)$ and a set of spatial augmentations $\Phi$, we can summarize CVRL objective as
% \begin{align}
% z_v = f_v(\phi(x))\\
% \mathcal{L}_v = \mathcal{L}(z_v^a, z_v^p, z_v^{n_i})
% \label{eq:lv}
% \end{align}
% where $\phi \in \Phi$ is an instance of a set of spatial augmentations. 
% $\mathcal{L}_v$ pulls together embedding $z_v^q$ and $z_v^k$ from the same video, while pushing away those from other videos ($z_v^{n_i}$). 

% This method pushes the network to learn good visual features since it needs to recognize different objects and scenes in the same video. However, it also naturally leads to temporal invariance since clips from the same video are forced to be similar in the embedding space even though they are extracted at different time points. This is sub-optimal for learning strong video representations especially when aiming at capturing temporal dynamics which are now rejected by the network.
% For example, ..... 
% \dvd{I would extend here with an actual example. For example, in a video with action XYZ, understanding the dynamics (NJD and FDS) helps... XXX. It's going to be a rather trivial example, but it will immediately make the reader understand the problem. We need to emphasise this more!}
%
\input{fig/targeted_sampling}
\subsection{Shuffled Contrastive Learning}
\label{sec:temporal_contrastive}
%
We address the problem of temporal invariance caused by CVRL by introducing our shuffled contrastive objective which is specifically targeted to extract motion information. 
For that, we produce positive pairs $x_{\scaleto{T}{4pt}}^a$ and $x_{\scaleto{T}{4pt}}^p$ by two independent spatial augmentations of the same clip from a video and the negatives  $x_{\scaleto{T}{4pt}}^{n_i}$ are created by shuffling the positive clip. 
This is key to our objective since the network cannot solve the task by looking at spatial clues, instead, we force it to pay attention to the temporal information inside the clips. 
To obtain a set of negatives, we apply a set of random permutations $\pi_i \in \Pi$ to the positive clip.
With that, our objective can be defined using a encoder $f_{\scaleto{T}{4pt}}$ as follows 
\begin{align}
\mathcal{L}_{\scaleto{T}{4pt}} = \mathcal{L}_{\text{contrastive}}(f_{\scaleto{T}{4pt}}; x_{\scaleto{T}{4pt}}^a, x_{\scaleto{T}{4pt}}^p, x_{\scaleto{T}{4pt}}^{n_i}).
\label{eq:lv}
\end{align}
The network can solve this objective only by being invariant to spatial augmentation and focus on temporal order which is the key to distinguish positives and negatives. Note, the different spatial augmentation between anchor and negative is crucial to avoid shortcuts, in fact without it a simple frame-by-frame comparison would solve the task easily without learning useful semantic information.
% Also, our method could fail in case there is not enough motion in the clip such that shuffling its frames actually produces a different looking clip. This is discussed in the next paragraph.
% The network can solve this objective only by being invariance to spatial augmentation (the difference between anchor and positive) and focus on temporal order which is the key to recognize positive and negative. Notice that the different spatial augmentation between anchor and negative is crucial to avoid shortcuts, in fact without it a simple frame-by-frame comparison would solve the task pretty easily without learning useful semantic information.
% Also, our method could fail in case there is not enough motion in the clip such that shuffling its frames actually produces a different looking clip. This is discussed in the next paragraph.
% \bb{Motivate why we need targeted sampling}
Sampling clips with low motion introduces ambiguous cases since shuffling their frames will generate almost the same clip, and thus same positive and negative samples. We propose a targeted sampling to tackle this issue.
\\
\noindent \textbf{Probabilistic targeted sampling.}
We aim to sample clips from video segments where there is high motion. To measure motion in a video, we utilize optical flow~\cite{brox-pami2011,weinzaepfel-iccv2013,flownet,teed-raft2020}. Yet, raw optical flow is sensitive to, e.g., global camera motion. That is why we use optical flow edges, following \cite{fanyi_modist}, to get a more robust estimate of foreground motion. These flow edges are created by applying a Sobel filter~\cite{sobel-sobel2014} onto the flow magnitude map. We take the median over the highest 4k flow edge pixels values in each frame and aggregate them in time by taking the median over all frames in a 1-second time window. 
This gives us a measure of motion strength for each 1-second window. 
Nevertheless, we also do not want to sample in a deterministic way the time step with the highest motion amplitude $m_t$ for each video, as that would exclude many useful training data. Instead, we sample the time step from a multinomial distribution according to weights $w_i$, which we obtain by inserting the motion amplitudes into the softmax function as
\begin{align}
    w_i = \sigma(m_i) =  \frac{e^{m_i / \beta}}{\sum_{j}^{T} e^{m_j / \beta}},
\label{eq:softmax}
\end{align}
with $\beta$ as the temperature regularizing the entropy of the distribution. 
Later in the experimental section we show the effect of this sampling on performances.
% \fy{This is confusing, we are sampling timestamps to shuffle, not different shuffles, right? but this equation is softmaxing over $N_T$ different shufflings}

\input{tab/architecture}
\subsection{Our SCVRL framework}
\noindent \textbf{Combine objectives.}
\label{sec:arch}
We train our self-supervised method by optimizing the combined losses as:
\begin{align}
    \mathcal{L} = \mathcal{L}_v + \lambda \mathcal{L}_t
\end{align}
with $\lambda$ as a weighting parameter. \fy{We can tone up a bit on this, texts are clear but doesn't make it sound interesting enough, we can make this a bigger deal...} To learn a common representation from both objectives, $\mathcal{L}_v$ and $\mathcal{L}_t$, we need to use a shared encoder.  Yet, both objectives are working against each other if minimized in the same representation space since $\mathcal{L}_v$ wants to pull all clips from the same video together while $\mathcal{L}_t$ wants to push them apart when shuffles. To circumvent that, we use a separate MLP head $\phi_{\cdot}$ for each objective which operates on top of a shared backbone $b$ with parameters $\theta_b$. With that, we can define the encoder for the visual contrastive loss as $f_v=\phi_v(b(\cdot))$ and similar for the temporal contrastive encoder $f_t=\phi_t(b(\cdot))$ with parameters $\theta_v$ and $\theta_t$ respectively. \\
\noindent \textbf{Architecture.}
We adopt a Multiscale Vision Transformer~\cite{MViT} (MViT) as our backbone, due to its large temporal receptive field, which makes it particularly suitable to learn from the proposed temporal contrastive learning objective. MViT operates on a feature hierarchy by progressively expanding the channel capacity, while reducing the feature resolution.
Each stage contains of multiple transformer blocks each consisting of Multi Head Pooling Attention (MHPA) to reduce computation in contrast to original Vision Transformers~\cite{dosovitskiy_vision_transformer_ICLR21} which uses Multi Head Attention. We use the MViT-Base (MViT-B) model which operates on videos of 16 frames. We provide an overview of the architecture in Tab.~\ref{table:arch}. As in previous work~\cite{MViT, arnab_vivit_2021} a cube projection layer is used to map the input video to tokens. This layer is implemented as a 3D convolution with a temporal kernel size of 3 and stride of 2 with padding of 1. Yet, when shuffling the input sequence, this projection layer would directly have access to the gaps between shuffled frames and would allow the network to learn shortcuts. That is why we shuffle groups of two frames and adapt the temporal kernel size to two with a stride of two to mitigate that. We ablate the importance of that in Tab.~\ref{table:ablation-kernel}.
\\
\noindent \textbf{Memory bank for efficiency.}
To effectively train our visual contrastive objective $\mathcal{L}_v$ we follow~\cite{wu-instdisc2018, he-moco2020} by constructing a memory bank of $N_v$ negative samples. For our temporal contrastive objective $\mathcal{L}_t$ negatives can be easily created by randomly permuting the query clip $N_t$ times. As suggested in \cite{he-moco2020}, we have a momentum and an online version of our full model with parameters $\theta = \{\theta_b, \theta_v, \theta_t\}$. The weights of the momentum version $\theta$ is regularly updated as a moving average of the online counterpart such as $\theta = m\theta + (1-m) \theta'$ with $m$ the momentum coefficient and $\theta'$ the parameters of the online model. We process the queries with our online model and the keys with the momentum version.










==> workshop/sec/4_results_bkup.tex <==
%!TEX root = ../main.tex
\section{Experiments}
\input{tab/architecture}

\subsection{Implementation Details}
\noindent \textbf{Training details.}
\bb{let's try to avoid implementation details already provided in previous papers. If you say "we follow ...." then we can skip everything they say, like the momentum part which is lengthy.}
We pretrain \ours{} on the Kinetics-400 (K400) dataset~\cite{kay-kinetics2017}, which contains around 240k 10-seconds videos, \textit{without} the use of the provided action annotations. 
To compare against the state-of-the-art, we pretrain \ours{} for 400 epochs, unless stated otherwise (e.g., 100 epochs in Tables \ref{table:diving} and \ref{table:ssv2}). For our ablation study we only train for 50 epochs on a subset of K400 containing 60k videos.  
To effectively train SCVRL with $\mathcal{L}^V$ we follow~\cite{wu-instdisc2018, he-moco2020} and construct a \emph{memory bank} of $N^V$ negative samples. To train with $\mathcal{L}^T$, instead, we generate negatives on the fly by randomly permuting the positive clip $N^T$ times. For the visual contrastive objective, we use a memory bank size $N^V$ of 65536 negative sample, while for the temporal counterpart we set $N_T=12$. For both objective we set the temperature $\tau$ to 0.1. \dvd{The next long paragraph about momentum still confuses me. Do we need it? If so, can we re-write it better?} As suggested in \cite{he-moco2020}, we have a momentum and an online version of our full model with parameters $\theta$. The weights of the momentum version $\theta$ is regularly updated as a moving average of the online counterpart such as $\theta = \lambda \theta + (1-\lambda) \theta'$ with $m$ the momentum coefficient and $\theta'$ the parameters of the online model. We process the queries with our online model and the keys with the momentum version. The momentum update is fixed to $\lambda=0.999$. The spatial augmentations are generated with random spatial cropping, temporal jittering, $p$ = 0.2 probability grayscale conversion, $p$ = 0.5 horizontal flip, $p$ = 0.5 Gaussian blur, and $p$ = 0.8 color perturbation on brightness, contrast and saturation, all with 0.4 jittering ratio. We train \ours{} with a learning rate of $1 \times 10^{-4}$ with linear warm-up and cosine annealing using Adamw optimizer~\cite{Loshchilov_adamw_ICLR2019} with a batch size of 4 per GPU and weight decay of $0.05$. We set the warm-up and end learning rate to $1\times 10^{-6}$.

\noindent \textbf{Architecture.} 
We use the \emph{MViT-Base} (MViT-B) version of MViT and operate on clips of 16 frames. Our architecture is shown Tab.~\ref{table:arch}. As in previous works~\cite{MViT, arnab_vivit_2021} a cube projection layer is used to map the input video to tokens. This layer is designed as a 3D convolution with a temporal kernel size of 3 and stride of 2 with padding of 1. However, when the input sequence is shuffled, the projection layer knows the gaps between shuffled frames and it could allow the network to learn shortcuts. To overcome this, we propose to shuffle groups of two frames and use a temporal kernel size to 2 with a stride of 2. Furthermore, each MLP head is a two-layer network that consists of a linear layer that transforms the CLS token to a 2048 dimensional feature vector, followed by a ReLU activation function, and a second linear layer that maps to an embedding of $128$-D.
\input{tab/diving}
\subsection{Evaluation Details}
\textbf{Evaluation protocol.} We follow previous works~\cite{qian-cvrl2020, recasens-brave2021} by employing two evaluation protocols to quantify self-supervised representations: (i) \textit{Linear}: Training a linear classification layer on top of the frozen pretrained backbone (ii) \textit{Full}: Fine-tuning the whole network in an end-to-end fashion on the target dataset. For all evaluations we report the top1 accuracy. \todo{Describe crops temporal spatial for inference}
\\
\noindent \textbf{Baselines.} We compare against (i) {\it CVRL}~\cite{qian-cvrl2020}, which is a state-of-the-art self-supervised contrastive learning method trained using the visual contrastive loss $\mathcal{L}^{V}$ of Eq.~\ref{eq:SCVRL} (with no explicit motion); and (ii) {\it Supervised}, which is a fully supervised model trained for action classification on K400. All baselines use the same MViT-B backbone as \ours{}.
\dvd{we need to think of a better way to present the results. it's a bit of a mass now. For example, we ablate on UCF (Table 5) before even presenting UCF. Do We need the distinction between spatial-heavy and temporal-heavy? I don't see any big result to motivate this split. What if we just present all the datasets and then all the results?}
\\
\textbf{Dataset}
\input{tab/ssv2}
\input{tab/low_shot_ssv2}
\input{tab/ucf}
% \input{tab/sota}


\subsection{Analysis of \ours{}}

\input{tab/drop}
\input{tab/ssv2_classes}
In this section we analyze the representations learned by \ours{} and compare them to the baseline CVRL.

\noindent \textbf{Dependence on motion information.}
In Tab.~\ref{table:shuffle_ablation} we analysis the dependence of temporal information on final performance for Diving-48 and UCF. Since both CVRL and \ours{} are trained without label annotations, we evaluate the linear fine-tuned model on the corresponding dataset. We follow previous works~\cite{MViT, sevilla_wacv_time_can_tell} and compare the performance difference between shuffling and non-shuffling the input during inference to evaluate temporal information learned. We observe that the performance drop from \ours{} is significant higher, around a factor of 3 for UCF and 1.8 for Diving-48. These results indicate that our model is much more sensitive to the temporal order of the frames and thus, consists of much more temporal aware features.
\input{tab/ablation}

\noindent \noindent \textbf{Performance comparison on SSv2.}
In Tab.~\ref{table:ssv2_comparison} we compare the performance of \ours{} on representative SSv2 classes to CVRL. For that, we use the models which are linear fine-tuned on SSv2 (see Tab. \ref{table:ssv2}). We observe that our model improves on classes wrt. to CVRL in which much motion occurs. To quantify the amount of motion for each class we compute the deviation in the pixel-space for each video and average them for all videos of one class. With that, we can clearly see that our model improves on classes in which strong motion is present. On the other hand, performance deteriorate on classes with very low motion such as "showing sth.". \ours{} improves significantly when looking at the overall performance difference. This experiment shows that \ours{} learns stronger motion sensitive features.

\noindent  \textbf{Video retrieval}
\todo{Add figure with video retrieval examples for \ours{} vs CVRL.} \michael{Planning to do on Sunday.}

\subsection{Comparison to state of the art}

In this section, we validate the effectiveness of \ours{} on common benchmarks for temporally heavy datasets, which are datasets which require the understanding of low-level motion cues.
Specifically, we evaluate our approach on two action classification datasets: Diving-48~\cite{diving-48} and  Something-Something-V2~\cite{ssv2}.

\paragraph{Action Classification on Diving-48}  
Diving-48 is a fine-grained action dataset capturing 48 unique diving classes. It has around 18k trimmed video clips each containing a diving sequence that consists of a mix of takeoff, the motion during the dive and water entering. It is a challenging dataset due to the semantic similarity across all diving classes (e.g., similar foreground and background, similar diving outfits, etc.), which makes it important to capture motion cues. Because of a problem with Diving-48 labels, we follow previous work~\cite{timesformer} and use the provided cleaned annotations.

\ours{} achieves the best performances of all self-supervised learning approaches for linear and full fine-tuning, which can be seen in Tab. \ref{table:diving}. Our proposed method even achieves similar performance than supervised for linear fine-tuning with around 16\% accuracy. We also compare our results to Timesformer~\cite{timesformer} which is a recent video transformer for video recognition. Timesformer evaluates their architecture after pre-training on ImageNet-1K in a supervised fashion. Similarly, they evaluate the SlowFast~\cite{slowfast} architecture. We observe that \ours{} effectively leverages the temporal data provided in Kinetics-400 and outperforms Timesformer-L as well as SlowFast even when only trained for 100 epochs. These results indicate that our proposed model effectively exploits temporal information provided in videos. \michael{too much?}

\paragraph{Action Classification on UCF and HMDB}
UCF101~\cite{soomro-ucf2012} and HMDB~\cite{kuehne-hmdb2011} are standard benchmarks for action classification representing sport activity and daily human actions. UCF contains 13320 YouTube videos categorized in 101 classes. HMDB consists of 6767 video clips and is divided into 51 categories. For all experiments on UCF101 and HMDB51, we report results using split1 for train/test split. 
\\
In \Table{ucf_hmdb} we show the top-1 accuracy on UCF and HMDB when fine-tuning the full network on each dataset after pre-training on Kinetics400. SCVRL outperforms its corresponding baseline CVRL by 2.4\% on UCF and 0.9\% on HMDB. This shows that even though that appearance cues are most important for these datasets, we still observe a performance gain compared to CVRL indicating that temporal sensitive features are also beneficial for those datasets. \michael{Should we also include linear numbers?}


\paragraph{Action Classification on SSv2}
Similarly to Diving-48, Something-Something-v2 is a benchmark that was specifically developed to evaluate a model's capability to capture dynamics. SSv2 consists of video clips showing complex human-object interactions, such as “Moving something up” and “Pushing something from left to right”, for a total of 174 actions. The train set contains 168K videos, an extra 24K videos are used for validation and 24K videos are available for testing. 
%open something and close something cannot be distinguished without reasoning across frames
\\
In \Table{ssv2} we compare different methods on this dataset using the same evaluation set-up as for Diving-48. We outperform other self-supervised approaches, with $1.5\%$ using the MViT-B architecture when fine-tuning the full model. For linear fine-tuning, we achieve performance on par with MoDist. We also compare our fully trained model with state-of-the-art self-supervised approaches. We improve upon these recent works and show that Vision Transformers are an effective backbone for self-supervised representation learning. \red{Needs to be adjusted if we achieve on par performance with supervised.} We are not able to directly compare with CORP~\cite{Hu_2021_ICCV_contrast_order} on SSv2 since they directly \textit{pretrain} on the target dataset which is an uncommon evaluation procedure in related works~\cite{}. We contacted the authors but code nor pretrained models could be provided. 

\paragraph{Low-shot learning on SSv2}
In \Table{lowshot} we evaluate our model in the context of low-shot learning, i.e. given only a fraction of the available train-set during fine-tuning. Both CVRL and \ours{} are pre-trained on the full Kinetics400 training set. The train-data ratio (top of the table) only applies to SSv2 fine-tuning. We perform the fine-tuning for 1\%, 5\%, 10\%, 25\%, 50\% and 100\% of SSv2 train data and show that SCVRL consistently outperforms CVRL by a significant margin. In particular, the relative gain of \ours{} is higher the lower the amount of data. This makes our proposed better suitable especially for target datasets with a lower amount of labeled data.


\subsection{Ablation studies}
In \Table{ablation-all} we provide detailed ablation studies on different components and design choices of our framework. For these studies we pretrain on the Kinetics-400 mini dataset and finetune for evaluation on UCF and SSv2.
\\
\textbf{Targeted sampling.} In Tab.~\ref{table:ablation-sampling} we evaluate the effect of our probabilistic targeted sampling on the final performance. We observe a performance boost with targeted sampling (temperature $\beta=5$) compared to uniform sampling (temperature $\beta = \infty$). Yet, for a low temperature in \Eq{softmax}, which corresponds to a low entropy of the distribution of weights $w_i$, we experience a lower performance. This might be caused by the fact that we exclude a lot of possible training data since most often the same clip is selected for the video. 

\noindent \textbf{Heads configuration.} We evaluate \ours{} with a single contrastive head $\phi_v=\phi_t$, which is shared for both objectives $\mathcal{L}^{V}$ and $\mathcal{L}^{T}$, and compare it to a model trained with separate heads, one for each objective. We observe in Tab.~\ref{table:ablation-heads} that minimizing both objectives in the same representation space hurts performance as it is even lower than for the model trained with $\mathcal{L}^V$ only. This confirm the necessity of using separate contrastive heads, as with it we see a clear performance gain to CVRL.  
% As discussed in Sec. \ref{sec:arch}, using a shared representation space for both objectives, ,  are defined as contrastive loss, a single head is sufficient for both tasks. However, we have developed a two-head approach (\Sec{arch}) which share the network back-bone. In \Table{ablation-heads} we compare the single-head approach "shared" and our final architecture "separate" and show that our approach achieves better performances.
\\
\textbf{Necessity of contrastive formulation.} In this ablation we compare our proposed objective $\mathcal{L}^T$ against a traditional pretext task approach~\cite{noroozi-iccv2017, brattoli-cvpr2017} based on a classifier trained using a cross-entropy loss to detect if a sequence is shuffled. This loss objective is combined with the visual contrastive objective $\mathcal{L}^T$ as in \ours{}. We observe in Tab.~\ref{table:ablation-components} that our proposed objective achieves much stronger performance for both UCF and SSv2, validating the importance of our novel framework.
% A classical implementation of shuffle task consists of a classification task with cross-entropy loss~\cite{brattoli-cvpr2017, noroozi-jigsaw2016}. We show that our adaptation with contrastive loss ("SCVRL") works much better than standard classification ("+ classifier shuffle") in the contest of video analysis (\Table{ablation-components}).
\\
\textbf{Used output feature representation.} We evaluate our proposed objective in \Table{ablation-representation} when trained on the output CLS token from MViT-B and compare it against using the output feature representation after applying average pooling over time and space. We obtain stronger results for the model which operates on the CLS token.
\\
\textbf{Shortcuts in projection layer.} We ablate the importance of our choice for the temporal kernel size in the projection layer. We experience in Tab.~\ref{table:ablation-kernel} that a model trained with a temporal kernel size $k_t$ of 3 performance better than a kernel size of 2, as can been seen in the first two rows. Yet, we observe a performance drop for \ours{} when trained with a kernel size of 3. In the latter the projection layer has directly access to the scenes between shuffled groups and can consequently reduce the temporal objective $\mathcal{L}^T$ using this shortcut. Thus, it is crucial for our framework to be trained with a kernel size which is aligned with the number of frames shuffled in each group. 


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.5\textwidth]{fig/ssv2_gainvsmotion.png}
%     \caption{
%     SCVRL gain relative to class motion. x-axis: class accuracy gain with and without our temporal loss $\mathcal{L}^T$; y-axis: video motion computed as at the end of \Sec{temporal_contrastive} and averaged over class.
%     There is a significant correlation between some high motion classes and the boost provided by our temporal loss, suggesting that the learned representation is related to motion.
%     }
%     \label{fig:method}
% \end{figure}

% \section{New Proposed Experiments structure}
% \begin{itemize}
%     \item Implementation details
%     \item Datasets
%     \item Shuffling frames during inference
%     \item Per class improvement related to motion
%     \item Low-shot learning on SSv2
%     \item comparison with state-of-the-art
%     \item Ablations
% \end{itemize}

==> workshop/sec/X_instructions.tex <==
%!TEX root = ../main.tex

% --- repeat the title (AT: haven't found a more elegant way to do this...)
\twocolumn[
\centering
\Large
\textbf{\LaTeX\ Author Guidelines for \confName~Proceedings (2022)}
\vspace{1.0em}
] %< twocolumn
\appendix

\setcounter{section}{0}
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of cvpr.sty to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the CVPR70 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.


% Update the cvpr.cls to do the following automatically.
% For this citation style, keep multiple citations in numerical (not
% chronological) order, so prefer \cite{Alpher03,Alpher02,Authors14} to
% \cite{Alpher02,Alpher03,Authors14}.


\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

%------------------------------------------------------------------------
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

%------------------------------------------------------------------------
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> workshop/sec/method_ckp1.tex <==
%!TEX root = ../main.tex
\section{Method}
\label{sec:method}
%
The goal of our approach is to better capture the temporal information inherent in videos in a self-supervised fashion. In Sec.~\ref{sec:visual_contrastive} we will first introduce a visual contrastive framework that yields robust spatial semantic features which acts as a strong baseline. Yet, it does not capture the temporal structures in videos. That is why we introduce in Sec.~\ref{sec:temporal_contrastive} our temporal contrastive objective to mitigate that. Lastly, in Sec.~\ref{sec:arch} we discuss our architecture and design choice for our framework. 
%
%
\subsection{Visual Contrastive Learning} 
\dvd{Baseline: VCL Objective}
\label{sec:visual_contrastive}
%
Recent work in self-supervised learning for images achieved impressive performance using contrastive learning~\cite{chen-simclr2020,he-moco2020,grill-byol2020}. This framework can be adapted for videos, as suggested in~\cite{qian-cvrl2020}, by adding temporal jitterring to the augmentations for the positive pairs , as visualized in Fig.~\ref{fig:method}. 
To be precise, given a randomly sampled query clip $c^q$ from an arbitrary video, we obtain its representation $z_v^q = f_v(\psi_1 (c^q))$ with an encoder $f_v$ and a temporally consistent spatial augmentation $\psi_1 \in \Psi$. Similar for the positive clip (key), we first randomly sample a second clip $c^k$ from the \textit{same} video and produce its representation $z_v^k = f_v(\psi_2 (c^k))$\joe{what is the spatial augmentation here?}. As negative samples we use 
$N$ clips $c^{n_i}$ with $i \in \{1,...,N_v\}$ from \textit{other} videos and obtain the corresponding embeddings $z^{n_i}_v = f_v(\psi_n (c^n_i))$. The visual contrastive framework is trained using the InfoNCE objective \cite{oord-arxiv2018,he-moco2020} 
\begin{align}
\mathcal{L}_{v} = -\log \frac{\exp(z_v^q {\cdot}z_v^k / \tau)}{\exp(z_v^q{\cdot}z_v^k / \tau) + \sum_{i}^{N_v}\exp(z_v^q{\cdot}z_v^{n_i}  / \tau)}, 
% \mathcal{L}_{v} = -\log \frac{e^{f_v(c^q)^T {\cdot}f_v(c^k) / \tau}}{e^{f_v(c^q)^T {\cdot}f_v(c^k) / \tau} + \sum_{i}^{N}e^{f_v(c^q)^T {\cdot}f_v(c^{n_i}) / \tau}}, 
\label{eq:lv}
\end{align}
%
with $\tau$ is a temperature hyperparameter. This objective pulls together embeddings $z_v^q$ and $z_v^k$ from the same video, while pushing away those from other videos. This naturally leads to temporal invariances since embeddings from the same video are forced to be similar. This is sub-optimal for learning strong video representations especially when aiming at capturing temporal dynamics.\dvd{I would extend here with an actual example. For example, in a video with action XYZ, understanding the dynamics (NJD and FDS) helps... XXX. It's going to be a rather trivial example, but it will immediately make the reader understand the problem. We need to emphasise this more!}
%
\subsection{Temporal Contrastive Learning}
\dvd{New TCL objective?}
\label{sec:temporal_contrastive}
%
We address the problem of temporal invariances by introducing our temporal contrastive objective. 
This objective aims to force the network to pay attention to the temporal order of the processed videos. 
We achieve this by applying contrastive learning on a set of positives and negatives that solely differ in their temporal content\joe{should find a different description than temporal content}, which is achieved by shuffling the video frames.
More specifically, we again obtain our representation for the query clip as $z_t^q = f_t(\psi_1 (c^q))$ using an encoder $f_t$.
Instead of using a clip from a different video, we apply a different set of augmentations $\psi_2 \in \Psi$ to the same clip $c^q$ to obtain the key representation $z_t^k = f_t(\psi_2 (c^q))$. \fy{are we going to use query/key vs anchor/positive?}
The embeddings of the negative clips are produced by shuffling the key clip $z_t^{n_i} = f_t(\pi_i (\psi_2 (c^q))), i \in \{1,...,N_t\}$ with $\pi_i \in \Pi$ a set of permutations to the video frames.
Similar to \eqref{eq:lv} we formulate our temporal contrastive framework as
\begin{align}
\mathcal{L}_{t} = -\log \frac{\exp(z_t^q {\cdot}z_t^k / \tau)}{\exp(z_t^q{\cdot}z_t^k / \tau) + \sum_{i}^{N_t}\exp(z_t^q{\cdot}z_t^{n_i} / \tau)}. 
\label{eq:lt}
\end{align}
By forcing the network to push apart embeddings from clips which only differ in their temporal order, we induce temporal information into the network. 
% \fy{One high level impression when reading both Sec. 3.1 and 3.2: we unnecessarily introduced many math notations, which are things could be explained well with plain English. I understand you want to make it looks more mathy, but I'm concerned readers might just be pissed when they figure out the notations are mostly just cluttering the description..}
\\

\noindent \textbf{Probabilistic targeted sampling.}
\joe{I feel this section is getting too in the weeds, maybe we should put it in implementation details on how to construct $\pi_i$ specific for a video.}
% To enhance the effectiveness of this objective, 
We aim to sample clips from video segments where there is high motion, as sampling clips with low motion introduces ambiguous cases which will hurt performance. To measure motion in a video, we utilize optical flow~\cite{brox-pami2011,weinzaepfel-iccv2013,flownet,teed-raft2020}. Yet, raw optical flow is sensitive to, e.g., global camera motion. That is why we use optical flow edges, following \cite{fanyi_modist}, to get a more robust estimate of foreground motion. These flow edges are created by applying a Sobel filter~\cite{sobel-sobel2014} onto the flow magnitude map. We take the median over the highest 4k flow edge pixels values in each frame and aggregate them in time by taking the median over all frames in a 1-second time window. 
This gives us a measure of motion strength for each 1-second window. 
Nevertheless, we also do not want to sample deterministically the time step with the highest motion amplitude $m_t$ for each video,  as that would exclude a lot of useful training data. Instead, we sample the time step from a multinomial distribution according to weights $w_i$, which we obtain by inserting the motion amplitudes into the softmax function as
\begin{align}
    w_i = \sigma(m_i) =  \frac{e^{m_i / \beta}}{\sum_{j}^{T} e^{m_j / \beta}},
\label{eq:softmax}
\end{align}
with $\beta$ as the temperature regularizing the entropy of the distribution. 
% \fy{This is confusing, we are sampling timestamps to shuffle, not different shuffles, right? but this equation is softmaxing over $N_T$ different shufflings}


\subsection{SCVRL Framework}
\label{sec:arch}
We train our self-supervised method by optimizing the combined losses as:
\begin{align}
    \mathcal{L} = \mathcal{L}_v + \lambda \mathcal{L}_t
\end{align}
with $\lambda$ as a weighting parameter. \fy{We can tone up a bit on this, texts are clear but doesn't make it sound interesting enough, we can make this a bigger deal...} To learn a common representation from both objectives, $\mathcal{L}_v$ and $\mathcal{L}_t$, we need to use a shared encoder.  Yet, both objectives are working against each if minimized in the same representation space since $\mathcal{L}_v$ wants to pull all clips from the same video together while $\mathcal{L}_t$ wants to push them apart if they are shuffled. To circumvent that, we use a separate MLP head $\phi_{\cdot}$ for each objective which operates on top of a shared backbone $b$ with parameters $\theta_b$. With that, we can define the encoder for the visual contrastive loss as $f_v=\phi_v(b(\cdot))$ and similar for the temporal contrastive encoder $f_t=\phi_t(b(\cdot))$ with parameters $\theta_v$ and $\theta_t$ respectively. \\
We adopt a Multiscale Vision Transformer~\cite{MViT} (MViT) as our backbone, due to its large temporal receptive field, which makes it particularly suitable to learn from the proposed temporal contrastive learning objective. MViT operates on a feature hierarchy by progressively expanding the channel capacity, while reducing the feature resolution.
Each stage contains of multiple transformer blocks each consisting of Multi Head Pooling Attention (MHPA) to reduce computation in contrast to original Vision Transformers~\cite{dosovitskiy_vision_transformer_ICLR21} which uses Multi Head Attention. We use the MViT-Base (MViT-B) model which operates on videos of 16 frames. We provide an overview of the architecture in Tab.~\ref{table:arch}. As in previous work~\cite{MViT, arnab_vivit_2021} a cube projection layer is used to map the input video to tokens. This layer is implemented as a 3D convolution with a temporal kernel size of 3 and stride of 2 with padding of 1. Yet, when shuffling the input sequence, this projection layer would directly have access to the gaps between shuffled frames and would allow the network to learn shortcuts. That is why we shuffle groups of two frames and adapt the temporal kernel size to two with a stride of two to mitigate that. We ablate the importance of that in Tab.~\ref{table:ablation-kernel}.
\\
\input{tab/architecture}
\noindent
To effectively train our visual contrastive objective $\mathcal{L}_v$ we follow~\cite{wu-instdisc2018, he-moco2020} by constructing a memory bank of $N_v$ negative samples. For our temporal contrastive objective $\mathcal{L}_t$ negatives can be easily created by randomly permuting the query clip $N_t$ times. As suggested in \cite{he-moco2020}, we have a momentum and an online version of our full model with parameters $\theta = \{\theta_b, \theta_v, \theta_t\}$. The weights of the momentum version $\theta$ is regularly updated as a moving average of the online counterpart such as $\theta = m\theta + (1-m) \theta'$ with $m$ the momentum coefficient and $\theta'$ the parameters of the online model. We process the queries with our online model and the keys with the momentum version.










==> workshop/tab/low_shot_diving.tex <==
\begin{table}[t]
\resizebox{\linewidth}{!}{
	\centering
	\small
	\begin{tabular}{l | c c c c c c}
		\multicolumn{1}{c|}{Method} 		& 1\% 		& 5\% 				& 10\% 			& 25\% 			& 50\% 			& 100\%
		\\
		\shline
    \demph{Rand Init}    &  \demph{6.8}   &  \demph{10.3}         & \demph{10.6}  & \demph{--}  & \demph{--}  & \demph{37.2}  
    \\
		\hline
		CVRL*  	& 7.4 & 15.4 & 27.6 & -- &-- & 83.1
		\\
		SCVRL 	& 8.3 & 16.4 & 27.7 & -- &-- & 84.7 
% 		\\
% 		\hspace{12pt}{$\Delta $} & +1.7		& +4.0	& +3.0	& +3.4	& +2.9	& +1.5	
		\\
		rel. $\Delta \%$ & +13.1 & +6.1 & +0.0 & +x.0 & +x.0 & +x.0
		
	\end{tabular}
	}
	\caption{\small  \textbf{Low-shot learning on Diving48.} Rows indicate different pretrainings on K400, while columns vary the \% of Diving48 training data used for finetuning. All results are top-1 accuracy. *: our implementation}
	\label{table:lowshot}
\vspace{-0.5cm}
\end{table}

==> workshop/tab/sota.tex <==
\setlength{\tabcolsep}{2pt}
\begin{table*}[!htb]
\footnotesize
  \centering
    \begin{tabular}{ll|ccccccc} 
    Method            & Date                & Dataset (duration)    & Architecture       & \hspace{6pt}Size        & \hspace{4pt}Modality  & Frozen      & UCF         & HMDB        \\ 
    \shline
    %     {Rand Init}        & \hspace{1pt}            & K400 (28d)          & MViT-B      & \hspace{6pt}224$^2$       & \hspace{4pt}V     & \cmark      & {??}      & {??}        \\
    % MoDist~\cite{fanyi_modist}        & 2021\hspace{1pt}            & K400 (28d)          & MViT-B      & \hspace{6pt}224$^2$       & \hspace{4pt}V     & \cmark      & {??}      & {??}        \\
    % {CVRL~\cite{fanyi_modist}}        & 2020\hspace{1pt}            & K400 (28d)          & MViT-B      & \hspace{6pt}224$^2$       & \hspace{4pt}V     & \cmark      & 82.0 & {54.6}        \\        
    % \rowcolor{GrayBG}
    % \textbf{\ours{}}        & \hspace{1pt}            & K400 (28d)          & MViT-B      & \hspace{6pt}224$^2$       & \hspace{4pt}V     & \cmark      & \textbf{84.4}      & \textbf{55.4}        \\
    % \demph{Supervised}        & \hspace{1pt}            & \demph{K400 (28d)}          & \demph{MViT-B}& \hspace{6pt}\demph{224$^2$}       & \hspace{4pt}\demph{V}     & \cmark      & \demph{??}      & \demph{??}        \\
    % \hline
    
    CBT~\cite{sun-cbt2019}    & 2019\hspace{1pt}          & K600+ (273d)        & S3D         & \hspace{6pt}112$^2$       & \hspace{4pt}V     & \cmark      & 54.0        & 29.5        \\
    MemDPC~\cite{han-memdpc2020}& 2020\hspace{1pt}          & K400 (28d)          & R-2D3D-34     & \hspace{6pt}224$^2$       & \hspace{4pt}V       & \cmark      & 54.1        & 30.5        \\
    MIL-NCE~\cite{miech-milnce2020}     & 2020\hspace{1pt}          & HTM (15y)           & S3D         & \hspace{6pt}224$^2$       & \hspace{4pt}V+T     & \cmark      & 82.7        & 53.1        \\
    MIL-NCE~\cite{miech-milnce2020}     & 2020\hspace{1pt}          & HTM (15y)           & I3D         & \hspace{6pt}224$^2$       & \hspace{4pt}V+T     & \cmark      & 83.4        & 54.8        \\
    XDC~\cite{alwassel-xdc2020}     & 2020\hspace{1pt}          & IG65M~(21y)         & R(2+1)D       & \hspace{6pt}224$^2$       & \hspace{4pt}V+A     & \cmark      & 85.3        & 56.0        \\ 
    ELO~\cite{piergiovanni-elo2020}   & 2020\hspace{1pt}          & Youtube8M (8y)        & R(2+1)D       & \hspace{6pt}224$^2$       & \hspace{4pt}V+A     & \cmark      & --        & 64.5        \\ 
    
    AVSlowFast~\cite{xiao-avslowfast2019} & 2020\hspace{1pt}          & K400 (28d)          & AVSlowFast-50 & \hspace{6pt}224$^2$     & \hspace{4pt}V+A       & \cmark      & {77.4}      & {42.2}      \\    

    CoCLR~\cite{han-coclr20}                & 2020\hspace{1pt}          & K400 (28d)          & S3D         & \hspace{6pt}128$^2$     & \hspace{4pt}V       & \cmark      & {74.5}      & {46.1}      \\    
    CVRL~\cite{qian-cvrl2020}       & 2021 \hspace{1pt}           & K400 (28d)          & R3D-50      & \hspace{6pt}224$^2$     & \hspace{4pt}V     & \cmark      & 89.8        & 58.3        \\ 
    BraVe~\cite{recasens-brave2021} & 2021 \hspace{1pt}           & K600 (36d)          & R3D-50      & \hspace{6pt}224$^2$     & \hspace{4pt}V     & \cmark      &  88.8        &  {\bf 61.8}        \\ 
    {CORP\cite{Hu_2021_ICCV_contrast_order}}      & 2021\hspace{1pt}            & K400 (28d)          & R3D-50      & \hspace{6pt}224$^2$       & \hspace{4pt}V       & \cmark      & {\bf 90.2}   & { 58.7}   \\
    % \textbf{MoDist\cite{fanyi_modist}}      & 2021\hspace{1pt}            & K400 (28d)          & R3D-50      & \hspace{6pt}224$^2$       & \hspace{4pt}V       & \cmark      & \textbf{91.5}   & \textbf{63.0}   \\
    \rowcolor{GrayBG}
    \textbf{\ours{}}      & \hspace{1pt}            & K400 (28d)          & MViT-B      & \hspace{6pt}224$^2$       & \hspace{4pt}V       & \cmark      & \textbf{??}   & \textbf{??}   \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \hline\hline
    % {Rand Init}        & \hspace{1pt}            & K400 (28d)          & MViT-B      & \hspace{6pt}224$^2$       & \hspace{4pt}V     & \xmark      & {??}      & {??}        \\
    % MoDist~\cite{fanyi_modist}        & 2021\hspace{1pt}            & K400 (28d)          & MViT-B      & \hspace{6pt}224$^2$       & \hspace{4pt}V     & \xmark      & {??}      & {??}        \\
    % {CVRL~\cite{fanyi_modist}}        & 2020\hspace{1pt}            & K400 (28d)          & MViT-B      & \hspace{6pt}224$^2$       & \hspace{4pt}V     & \xmark      & 82.0 & {54.6}        \\        
    % \rowcolor{GrayBG}
    % \textbf{\ours{}}        & \hspace{1pt}            & K400 (28d)          & MViT-B      & \hspace{6pt}224$^2$       & \hspace{4pt}V     & \xmark      & \textbf{84.4}      & \textbf{55.4}        \\
    % \demph{Supervised}        & \hspace{1pt}            & \demph{K400 (28d)}          & \demph{MViT-B}& \hspace{6pt}\demph{224$^2$}       & \hspace{4pt}\demph{V}     & \xmark     &  93.4 & 68.8 \\
    % \hline
    {Rand Init}    &                   & \hspace{12pt}{-}  & {R3D-50}  & \hspace{6pt}\demph{224$^2$} & \hspace{4pt}{V} & {\xmark}  & {69.0}    & {22.7}    \\ 
    OPN~\cite{lee-iccv2017}         & 2017\hspace{1pt}            & UCF (1d)            & VGG         & \hspace{6pt}227$^2$       & \hspace{4pt}V     & \xmark      & 59.6        & 23.8        \\ 
    3D-RotNet~\cite{jing-arxiv2018}   & 2018\hspace{1pt}            & K400 (28d)          & R3D-18      & \hspace{6pt}112$^2$       & \hspace{4pt}V     & \xmark      & 62.9        & 33.7        \\ 
    ST-Puzzle~\cite{kim-aaai2019}   & 2019\hspace{1pt}            & K400 (28d)          & R3D-18      & \hspace{6pt}224$^2$       & \hspace{4pt}V     & \xmark      & 63.9        & 33.7        \\ 
    VCOP~\cite{xu-vcop2019}     & 2019\hspace{1pt}            & UCF (1d)            & R(2+1)D       & \hspace{6pt}112$^2$       & \hspace{4pt}V     & \xmark      & 72.4        & 30.9        \\ 
    DPC~\cite{han-dpc2019}          & 2019 \hspace{1pt}           & K400 (28d)          & R-2D3D-34     & \hspace{6pt}128$^2$       & \hspace{4pt}V     & \xmark      & 75.7        & 35.7        \\ 
    CBT~\cite{sun-cbt2019}          & 2019\hspace{1pt}            & K600+ (273d)        & S3D         & \hspace{6pt}112$^2$       & \hspace{4pt}V     & \xmark      & 79.5        & 44.6        \\
    DynamoNet~\cite{diba-dynamonet2019}   & 2019\hspace{1pt}            & Youtube8M-1 (58d)       & STCNet      & \hspace{6pt}112$^2$       & \hspace{4pt}V     & \xmark      & 88.1        & 59.9        \\ 
    AVTS~\cite{korbar-nips2018}     & 2018\hspace{1pt}            & K400 (28d)          & I3D         & \hspace{6pt}224$^2$       & \hspace{4pt}V+A     & \xmark      & 83.7        & 53.0        \\
    AVTS~\cite{korbar-nips2018}     & 2018 \hspace{1pt}           & AudioSet (240d)       & MC3         & \hspace{6pt}224$^2$       & \hspace{4pt}V+A     & \xmark      & 89.0        & 61.6        \\
    XDC~\cite{alwassel-xdc2020}     & 2019  \hspace{1pt}          & K400~(28d)          & R(2+1)D       & \hspace{6pt}224$^2$       & \hspace{4pt}V+A     & \xmark      & 84.2        & 47.1        \\ 
    XDC~\cite{alwassel-xdc2020}     & 2019  \hspace{1pt}          & IG65M~(21y)         & R(2+1)D       & \hspace{6pt}224$^2$       & \hspace{4pt}V+A     & \xmark      & 94.2        & 67.4        \\ 
    AVSlowFast~\cite{xiao-avslowfast2019} & 2020\hspace{1pt}          & K400 (28d)          & AVSlowFast-50 & \hspace{6pt}224$^2$     & \hspace{4pt}V+A       & \xmark      & {87.0}      & {54.6}      \\    
    SpeedNet~\cite{benaim-speednet2020}   & 2020 \hspace{1pt}           & K400 (28d)          & S3D-G       & \hspace{6pt}224$^2$       & \hspace{4pt}V     & \xmark      & 81.1        & 48.8        \\
    MemDPC~\cite{han-memdpc2020}  &2020\hspace{1pt}           & K400 (28d)          & R-2D3D-34     & \hspace{6pt}224$^2$       & \hspace{4pt}V     & \xmark      & 86.1        & 54.5        \\
    CoCLR~\cite{han-coclr20}  &  \hspace{1pt}2020         & K400 (28d)          & S3D         & \hspace{6pt}128$^2$       & \hspace{4pt}V       & \xmark      & {87.9}      & {54.6}        \\
    GDT~\cite{patrick-gdt2020}      & 2020 \hspace{1pt}           & K400 (28d)          & R(2+1)D       & \hspace{6pt}112$^2$       & \hspace{4pt}V+A     & \xmark      & 89.3        & 60.0        \\ 
    GDT~\cite{patrick-gdt2020}      & 2020 \hspace{1pt}           & IG65M~(21y)         & R(2+1)D       & \hspace{6pt}112$^2$       & \hspace{4pt}V+A     & \xmark      & 95.2        & 72.8        \\ 
    MIL-NCE~\cite{miech-milnce2020}   & 2020\hspace{1pt}            & HTM (15y)           & S3D         & \hspace{6pt}224$^2$       & \hspace{4pt}V+T     & \xmark      & 91.3        & 61.0        \\
    ELO~\cite{piergiovanni-elo2020}   & 2020\hspace{1pt}          & Youtube8M-2 (13y)       & R(2+1)D       & \hspace{6pt}224$^2$       & \hspace{4pt}V+A     & \xmark      & 93.8        & 67.4        \\ 
    CVRL~\cite{qian-cvrl2020}       & 2021 \hspace{1pt}           & K400 (28d)          & R3D-50      & \hspace{6pt}224$^2$     & \hspace{4pt}V     & \xmark      & 92.9        & 67.9        \\ 
    BraVe~\cite{recasens-brave2021} & 2021 \hspace{1pt}           & K600 (36d)          & R3D-50      & \hspace{6pt}224$^2$     & \hspace{4pt}V     & \xmark      &  92.6        &  {\bf 69.2}        \\ 
    CORP\cite{Hu_2021_ICCV_contrast_order}        & 2021\hspace{1pt}            & K400 (28d)          & R3D-50      & \hspace{6pt}224$^2$       & \hspace{4pt}V       & \xmark      & {\bf 93.5}      & { 68.0}        \\
    % MoDist\cite{fanyi_modist}        & 2021\hspace{1pt}            & K400 (28d)          & R3D-50      & \hspace{6pt}224$^2$       & \hspace{4pt}V       & \xmark      & {\bf 94.0}      & { 67.4}        \\
    % MoDist\cite{fanyi_modist}        & 2021\hspace{1pt}          & K400 (28d)          & R3D-50      & \hspace{6pt}224$^2$       & \hspace{4pt}V+F     & \xmark      & { 94.2}      & { 67.3}        \\
        \rowcolor{GrayBG}
    \textbf{\ours{}}        & \hspace{1pt}            & K400 (28d)          & MViT-B      & \hspace{6pt}224$^2$       & \hspace{4pt}V     & \xmark      & {??}      & {??}        \\
    \demph{Supervised}        & \hspace{1pt}            & \demph{K400 (28d)}          & \demph{S3D}& \hspace{6pt}\demph{224$^2$}       & \hspace{4pt}\demph{V}     & \xmark       & \demph{96.8}    & \demph{75.9}      \\
    \hline
    \end{tabular}
  \caption{\small \textbf{Comparison with state-of-the-art approaches.}
    We report top-1 accuracy in this table.
    In parenthesis, we show the total video duration in time (\textbf{d} for day, \textbf{y} for year).
    Top half of the table contains results for Linear protocol (Frozen \cmark), whereas the bottom half shows results for the Full end-to-end finetuning protocol (Frozen \xmark).  
    For modality, V refers to visual only, A is audio, T is text narration. 
    We computed the results for \ours{} and variants and also the ``w/o Pretrain'' entry. Other entries are taken from their respective paper.
    }
  \label{table:sota-classification}
\end{table*}

